Quantum Simulation of non-Abelian Lattice Gauge Theories: a variational approach to $\mathbb{D}_8$

In this work, we address the problem of a resource-efficient formulation of non-Abelian LGTs by focusing on the difficulty of simulating fermionic degrees of freedom and the Hilbert space redundancy. First, we show a procedure that removes the matter and improves the efficiency of the hardware resources. We demonstrate it for the simplest non-Abelian group addressable with this procedure, $\mathbb{D}_8$, both in the cases of one (1D) and two (2D) spatial dimensions. Then, with the objective of running a variational quantum simulation on real quantum hardware, we map the $\mathbb{D}_8$ lattice gauge theory onto qudit systems with local interactions. We propose a variational scheme for the qudit system with a local Hamiltonian, which can be implemented on a universal qudit quantum device as the one developed in $\href{https://doi.org/10.1038/s41567-022-01658-0}{[Nat. Phys. 18, 1053 (2022)]}$. Our results show the effectiveness of the matter-removing procedure, solving the redundancy problem and reducing the amount of quantum resources. This can serve as a way of simulating lattice gauge theories in high spatial dimensions, with non-Abelian gauge groups, and including dynamical fermions.

==> Sections/test_material.tex <==
\begin{table}[h]
  \begin{tabular}{|c|c|}
        \multicolumn{2}{c}{\textbf{Clebsch-Gordan Coefficients and Related Values}} \\
        \hline
        Coefficients & Value \\
        \hline
        $ \braket{0|00}, \qquad \braket{0|\Bar{0}\Bar{0}}, \qquad \braket{0|11}, \qquad \braket{0|\Bar{1}\Bar{1}}$ & 1 \\ 
        $ \braket{\Bar{0}|\Bar{0}0}, \qquad \braket{\Bar{0}|0\Bar{0}}, \qquad \braket{\Bar{0}|1\Bar{1}}, \qquad \braket{\Bar{0}|\Bar{1}1}$ & 1 \\ 
        $ \braket{1|10}, \qquad \braket{1|01}, \qquad \braket{1|\Bar{0}\Bar{1}}, \qquad \braket{1|\Bar{1}\Bar{0}}$ & 1 \\
        $ \braket{\Bar{1}|\Bar{1}0}, \qquad \braket{\Bar{1}|0\Bar{1}}, \qquad \braket{\Bar{1}|\Bar{0}1}, \qquad \braket{\Bar{1}|1\Bar{0}}$ & 1 \\ 
        $ \braket{0,2m|2m'}, \qquad \braket{2m, 0|2m'}$ & $\delta_{m,m'}$ \\ 
        $ \braket{\Bar{0},2m|2m'}, \qquad \braket{2m, \Bar{0}|2m'}$ & $\varepsilon_{m,m'}$ \\ 
        $ \braket{1,2m|2m'}, \qquad \braket{2m, 1|2m'}$ & $(\sigma_z)_{m,m'}$ \\ 
        $ \braket{\Bar{1},2m|2m'}, \qquad \braket{2m, \Bar{1}|2m'}$ & $(\sigma_x)_{m,m'}$ \\ 
        \hline
        \multicolumn{2}{c}{} \\ % Spazio tra le sezioni
        \multicolumn{2}{c}{\textbf{Clebsch-Gordan Coefficients for $m, m' \in \{0,1\}$}} \\
        \hline
        Coefficients & $(m,m') = (0,0), (0,1), (1,0), (1,1)$ \\
        \hline
        $ \braket{0|2m, 2m'} = Q^0_{m,m'}$ & $\dfrac{1}{\sqrt{2}}(1, 0, 0, 1)$ \\ 
        $ \braket{\Bar{0}|2m, 2m'} = Q^{\Bar{0}}_{m,m'}$ & $\dfrac{1}{\sqrt{2}}(0, 1, -1, 0)$ \\ 
        $ \braket{1|2m, 2m'} = Q^1_{m,m'}$ & $\dfrac{1}{\sqrt{2}}(1, 0, 0, -1)$ \\ 
       $ \braket{\Bar{1}|2m, 2m'} = Q^{\Bar{1}}_{m,m'}$ & $\dfrac{1}{\sqrt{2}}(0, 1, 1, 0)$ \\ 
        \hline
    \end{tabular}
    \caption{Clebsch-Gordan Coefficients, $m, m' \in \{0,1\}$. CG coefficients were computed using the Clebsch-Gordan series \cite{brink1994angular}: $D^{j_1}_{m_1m_1'} D^{j_2}_{m_2m_2'} = \sum_J \braket{j_1m_1j_2m_2|JM} \braket{JM'|j_1m_1'j_2m_2'}D^J_{MM'}$. }
    \label{C-G coeff}
 \end{table}

==> figures/matrix_hamiltonian_after.tex <==
\begin{figure}
    \centering
\[ H^{(2)} = \scalebox{0.7}{ 
\begin{bmatrix}
  2M & 0 & 0 &  0 & 0 & 0 & 0 & -iJ \sqrt{2} & 0 & 0\\
  0 & 2M & 0 & 0 & 0 & 0 & 0 & 0 & 0 & iJ \sqrt{2} \\
  0 & 0 & 2M & 0 & 0 & 0 & 0 & 0 & iJ \sqrt{2} & 0\\
  0 & 0 & 0  & -2M & 0 & 0 & 0 & -iJ \sqrt{2} & iJ \sqrt{2} & iJ \sqrt{2}\\
  0 & 0 & 0  & 0   & M + 2\lambda_E& 0 & 0 & iJ & 0 & -iJ\\
  0 & 0 & 0  &   0 &  0  &  M + 2\lambda_E & 0 & iJ & -iJ & 0\\
  0 & 0 & 0  &  0  &  0  &  0  &   M + 2\lambda_E & 0 & iJ & iJ\\
  iJ \sqrt{2} & 0 & 0  &  iJ \sqrt{2}  &  -iJ  &  -iJ  &  0  &  \lambda_E & 0 & 0\\
  0 & 0 & -iJ \sqrt{2}  & -iJ \sqrt{2}   &  0 & iJ  &  -iJ  &  0  & \lambda_E & 0\\
  0 & -iJ \sqrt{2} & 0  &  -iJ \sqrt{2}  &  iJ  & 0   & -iJ   & 0   &  0  &   \lambda_E \\
  \label{matrix_without_matter}
\end{bmatrix}}
\]
 \caption{Transformed Hamitonian evaluated over the transformed gauge invariant states.} %We can observe that it is similar to the one obtained in \ref{Matrix_with_matter}.}
  \label{Matrix_without_matter}
\end{figure}

==> figures/matrix_hamiltonian_before.tex <==
\begin{figure}[h]
    \centering
\[ H = 
\scalebox{0.75}{\begin{bmatrix}
  2M & 0 & 0 &  0 & 0 & 0 & 0 & -J \sqrt{2} & 0 & 0\\
  0 & 2M & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -J \sqrt{2} \\
  0 & 0 & 2M & 0 & 0 & 0 & 0 & 0 & -J \sqrt{2} & 0\\
  0 & 0 & 0  & -2M & 0 & 0 & 0 & -J \sqrt{2} & -J \sqrt{2} & -J \sqrt{2}\\
  0 & 0 & 0  & 0   & M + 2\lambda_E& 0 & 0 & -J & 0 & -J\\
  0 & 0 & 0  &   0 &  0  &  M + 2\lambda_E & 0 & -J & -J & 0\\
  0 & 0 & 0  &  0  &  0  &  0  &   M + 2\lambda_E & 0 & -J & -J\\
  -J \sqrt{2} & 0 & 0  &  -J \sqrt{2}  &  -J  &  -J  &  0  &  \lambda_E & 0 & 0\\
  0 & 0 & -J \sqrt{2}  & -J \sqrt{2}   &  0 & -J  &  -J  &  0  & \lambda_E & 0\\
  0 & -J \sqrt{2} & 0  &  -J \sqrt{2}  &  -J  & 0   & -J   & 0   &  0  &   \lambda_E
\end{bmatrix}}
\]    \caption{Original Hamitonian evaluated over the ten gauge invariant states.}
  \label{Matrix_with_matter}
\end{figure}
